DenoDet V2: Phase-Amplitude Cross Denoising for SAR Object Detection

One of the primary challenges in Synthetic Aperture Radar (SAR) object detection lies in the pervasive influence of coherent noise. As a common practice, most existing methods, whether handcrafted approaches or deep learning-based methods, employ the analysis or enhancement of object spatial-domain characteristics to achieve implicit denoising. In this paper, we propose DenoDet V2, which explores a completely novel and different perspective to deconstruct and modulate the features in the transform domain via a carefully designed attention architecture. Compared to DenoDet V1, DenoDet V2 is a major advancement that exploits the complementary nature of amplitude and phase information through a band-wise mutual modulation mechanism, which enables a reciprocal enhancement between phase and amplitude spectra. Extensive experiments on various SAR datasets demonstrate the state-of-the-art performance of DenoDet V2. Notably, DenoDet V2 achieves a significant 0.8\% improvement on SARDet-100K dataset compared to DenoDet V1, while reducing the model complexity by half. The code is available at https://github.com/GrokCV/GrokSAR.

==> arxiv_contents/1-authors.tex <==
% !TEX root = ../main_arxiv.tex

% author names and IEEE memberships
\author{
  Kang~Ni,
  Minrui~Zou,
  Yuxuan~Li,
  Xiang~Li,
  Kehua~Guo,
  Jian~Yang,
  Ming-Ming Cheng,
  Yimian~Dai
  \thanks{
    This work was supported by
      % 国家自然科学基金
      the National Natural Science Foundation of China (62101280, % 倪康师弟
      62301261, % 我
      62206134, % 翔哥      
      % 62472443, % 郭克华老师
      U24A20330, 62361166670), % 杨健老师
    % 博后面上
    the Fellowship of China Postdoctoral Science Foundation (2023M731781). % 倪康
    % , 
    % 2021M701727). % 我
    \emph{(Corresponding authors: Yimian Dai.)
    }
  }

  % 南邮
\thanks{
  Kang Ni and Minrui Zou are
  % , and Zhizhong Zheng are 
  with Nanjing University of Posts and Telecommunications, Nanjing, China. Kang Ni is also with Key Laboratory of Radar Imaging and Microwave Photonics, Nanjing University of Aeronautics and Astronautics, Ministry of Education, Nanjing, China.
  (e-mail:
  \href{mailto:tznikang@163.com}{tznikang@163.com};
  \href{mailto:traveler\_wood@163.com}{traveler\_wood@163.com}).
  % \href{mailto:zhengzz\_js@126.com}{zhengzz\_js@126.com}
  
}

  % 南开
  \thanks{
  Yuxuan Li, Xiang Li, Jian Yang, and Yimian Dai are with VCIP, College of Computer Science, Nankai University. 
  Xiang Li also holds a position at the NKIARI, Shenzhen Futian. 
  (e-mail:
  \href{mailto:yuxuan.li.17@ucl.ac.uk}{yuxuan.li.17@ucl.ac.uk};
  \href{mailto:xiang.li.implus@nankai.edu.cn}{xiang.li.implus@nankai.edu.cn};
  \href{mailto:csjyang@nankai.edu.cn}{csjyang@nankai.edu.cn};
  \href{mailto:yimian.dai@gmail.com}{yimian.dai@gmail.com})
  }

  % 中南
  % \thanks{
  %   Kehua Guo is affiliated with School of Computer Science and Engineering, Central South University, Changsha 410083, China.
  %   (e-mail: \href{mailto:guokehua@csu.edu.cn}{guokehua@csu.edu.cn}).
  % }
  
  % 南理工
  % \thanks{
  %    Jian Yang and Yimian Dai are with PCA Lab, Key Lab of Intelligent Perception and Systems for High-Dimensional Information of Ministry of Education, and Jiangsu Key Lab of Image and Video Understanding for Social Security, School of Computer Science and Engineering, Nanjing University of Science and Technology, Nanjing, China.
  %   (e-mail:
  %   \href{mailto:csjyang@njust.edu.cn}{csjyang@mail.njust.edu.cn};
  %   \href{mailto:yimian.dai@gmail.com}{yimian.dai@gmail.com}).
  % }
}


==> arxiv_contents/2-abstract.tex <==
% !TEX root = ../main_arxiv.tex

\begin{abstract}
One of the primary challenges in Synthetic Aperture Radar (SAR) object detection lies in the pervasive influence of coherent noise.
As a common practice, most existing methods, whether handcrafted approaches or deep learning-based methods, employ the analysis or enhancement of object spatial-domain characteristics to achieve implicit denoising.
In this paper, we propose DenoDet V2, which explores a completely novel and different perspective to deconstruct and modulate the features in the transform domain via a carefully designed attention architecture.
% This ``Attention as Feature Denoising'' paradigm is inspired and introduced in DenoDet V1, which offers an interpretation of attention mechanisms as frequency-domain dynamic soft threshold shrinkage operations.
Compared to DenoDet V1, DenoDet V2 is a major advancement that exploits the complementary nature of amplitude and phase information through a band-wise mutual modulation mechanism, which enables a reciprocal enhancement between phase and amplitude spectra.
Extensive experiments on various SAR datasets demonstrate the state-of-the-art performance of DenoDet V2. Notably, DenoDet V2 achieves a significant 0.9\% improvement on SARDet-100K dataset compared to DenoDet V1, while reducing the model complexity by half.
% The code is available at \url{https://github.com/GrokCV/GrokSAR}.
The code will be available soon.

% Synthetic Aperture Radar (SAR) target detection plays a crucial role in various applications, but it faces challenges due to the presence of small targets and speckle noise.
% Although recent deep learning-based methods have made significant progress by incorporating frequency-domain information, they often process amplitude and phase in isolation and suffer from increased model complexity and over-interaction. 
% In this paper, we propose DenoDet V2, a novel approach that exploits the complementary nature of amplitude and phase information through a mutual guidance mechanism. Central to our method is the Phase-Amplitude Token Exchange (PATE) module, which enables a reciprocal enhancement between phase and amplitude spectra, resulting in a synergistic feature denoising effect. 
% Furthermore, we introduce a localized, band-specific denoising approach that ensures fine-grained noise suppression while preserving critical spatial and structural information. 
% Extensive experiments on various SAR datasets demonstrate the state-of-the-art performance of DenoDet V2, showcasing its potential for robust and precise target detection in noisy SAR environments.
% The code is available at \url{https://github.com/GrokCV/GrokSAR}.

\end{abstract}
% \vspace{-1\baselineskip}

==> arxiv_contents/9-biography.tex <==
% !TEX root = ../main_arxiv.tex

% Kang Ni
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Kang-Ni}}]{Kang Ni (Member, IEEE) } received the M.S. degrees from Changchun University of Technology, Jilin, China, in 2016, and the Ph.D. degree from Nanjing University of Aeronautics and Astronautics, Jiangsu, China, in 2020.
He is an Associate Professor with the School of Computer Science, Nanjing University of Posts and Telecommunications, Nanjing, and also a member with the Jiangsu Key Laboratory of Big Data Security and Intelligent Processing, Nanjing. His research interests include machine learning, SAR image processing, and computer vision.
\end{IEEEbiography}

% Minrui Zou
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Minrui-Zou-Crop}}]{Minrui Zou} received the B.E. degree from the Civil Aviation University of China, Tianjin, China, in 2022. And he is pursuing the M.S. degree in the School of Computer Science, Nanjing University of Posts and Telecommunications, Jiangsu, China. His research interests include machine learning and computer vision.
\end{IEEEbiography}

% Zhizhong Zheng
% \begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Zhizhong-Zheng}}]{Zhizhong Zheng} received the B.S degree in electronic engineering from the Jilin University, Changchun, China, in 2001, and the Ph.D. degree in Control Engineer from the Nanjing University of Aeronautics and Astronautics (NUAA), Nanjing, China, in 2021, respectively. He has developed a series of equipments such as space remote sensing camera, airbone hyperspectral imaging instrument, UAV hyperspectral remote sensing system, little field spectrometer, and core scan spectral imaging system, as well as spectral data processing and information extraction software. Now he is a team leader of Hyperspectral Remote Sensing and Intelligent Perception of the Nanjing University of Posts and Telecommunications (NJUPT).
% \end{IEEEbiography}

% Yuxuan Li
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Yuxuan-Crop}}]{Yuxuan Li} is currently a Ph.D. student at the Department of Computer Science, Nankai University, China.
  He graduated from University College London (UCL) with a first-class degree in Computer Science. He was the champion of the Second Jittor Artificial Intelligence Challenge in 2022, was awarded 2nd place in Facebook Hack-a-Project in 2019 and was awarded 2nd place in the Greater Bay Area International Algorithm Competition in 2022. His research interests include neural architecture design, and remote sensing object detection. 
\end{IEEEbiography}

% Yulei Qian
% \begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Yulei_Qian}}]{Yulei Qian} received his PhD degree from College of Electronic and Information Engineering, Nanjing University of Aeronautics and Astronautics in 2020. He is now an engineer in Nanjing Marine Radar Institute. His main research interests include target detection, radar imaging, satellite synthetic aperture radar, sparse recovery, deconvolution and radar waveform design. He has published 10+ paper in remote sensing journals and conferences.
% \end{IEEEbiography}

% Xiang Li
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Xiang_Li}}]{Xiang Li} is an Associate Professor in College of Computer Science, Nankai University. He received the PhD degree from the Department of Computer Science and Technology, Nanjing University of Science and Technology (NJUST) in 2020. There, he started the postdoctoral career in NJUST as a candidate for the 2020 Postdoctoral Innovative Talent Program. In 2016, he spent 8 months as a research intern in Microsoft Research Asia, supervised by Prof. Tao Qin and Prof. Tie-Yan Liu. He was a visiting scholar at Momenta, mainly focusing on monocular perception algorithm. His recent works are mainly on: neural architecture design, CNN/Transformer, object detection/recognition, unsupervised learning, and knowledge distillation. He has published 20+ papers in top journals and conferences such as TPAMI, CVPR, NeurIPS, etc.
\end{IEEEbiography}

% Kehua Guo
% \begin{IEEEbiography}[{
% \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Kehua-Guo}}]{Kehua Guo} Kehua Guo (M'13) received the Ph.D. degree in Computer Science and Technology from Nanjing University of Science and Technology, Nanjing, China, in 2008. He is currently a professor with Central South University, Changsha, China. He has served as a Guest Editor, Workshop Chair, Publicity Chair, Technical Program Committee Member, and Reviewer of international journals/conference proceedings. His research interests include artificial intelligence, big data, and image processing.
% \end{IEEEbiography}


% Jian Yang
\begin{IEEEbiography}[{
  \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Jian_Yang}}]{Jian Yang} received the PhD degree from Nanjing University of Science and Technology (NJUST) in 2002, majoring in pattern recognition and intelligence systems. From 2003 to 2007, he was a Postdoctoral Fellow at the University of Zaragoza, Hong Kong Polytechnic University and New Jersey Institute of Technology, respectively. From 2007 to present, he is a professor in the School of Computer Science and Technology of NJUST. Currently, he is also a visiting distinguished professor in the College of Computer Science of Nankai University. His papers have been cited over 50000 times in the Google Scholar. His research interests include pattern recognition and computer vision. Currently, he is/was an associate editor of Pattern Recognition, Pattern Recognition Letters, IEEE Trans. Neural Networks and Learning Systems, and Neurocomputing. He is a Fellow of IAPR.
\end{IEEEbiography}



% Yimian Dai
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Yimian_Dai}}]{Yimian Dai} 
(Member, IEEE) received the B.E. degree in information engineering and the Ph.D. degree in signal and information processing from Nanjing University of Aeronautics and Astronautics, Nanjing, China, in 2013 and 2020, respectively.
From 2021 to 2024, he was a Postdoctoral Researcher with the School of Computer Science and Engineering, Nanjing University of Science and Technology, Nanjing, China. 
He is currently an Associate Professor with the College of Computer Science, Nankai University, Tianjin, China.
His research interests include computer vision, deep learning, and their applications in remote sensing.
For more information, please visit the link (\href{https://yimian.grokcv.ai/}{https://yimian.grokcv.ai/}).
% (Member, IEEE) received the B.S. and Ph.D. degrees in signal and information processing from Nanjing University of Aeronautics and Astronautics (NUAA), Nanjing, China, in 2013 and 2021, respectively.
% From 2021 to 2024, he was a Postdoctoral Researcher with the School of Computer Science and Engineering, Nanjing University of Science and Technology (NJUST), Nanjing, China. During his Ph.D. study, he was a visiting scholar at the Department of Computer Science, University of Copenhagen, Denmark, under the supervision of Prof. Fabian Gieseke from March 2018 to September 2018, and at the Department of Computer Science, University of Arizona, USA, under the supervision of Prof. Kobus Barnard from October 2018 to October 2020.

% Since 2025, he has been an Associate Professor with the College of Computer Science, Nankai University, Tianjin, China. His research interests include computer vision, deep learning, and their applications in remote sensing, with a particular focus on developing advanced object detection algorithms to address real-world challenges.
\end{IEEEbiography}
